Structured Mixture of Continuation-ratio Logits Models for Ordinal Regression

We develop a nonparametric Bayesian modeling approach to ordinal regression based on priors placed directly on the discrete distribution of the ordinal responses. The prior probability models are built from a structured mixture of multinomial distributions. We leverage a continuation-ratio logits representation to formulate the mixture kernel, with mixture weights defined through the logit stick-breaking process that incorporates the covariates through a linear function. The implied regression functions for the response probabilities can be expressed as weighted sums of parametric regression functions, with covariate-dependent weights. Thus, the modeling approach achieves flexible ordinal regression relationships, avoiding linearity or additivity assumptions in the covariate effects. Model flexibility is formally explored through the Kullback-Leibler support of the prior probability model. A key model feature is that the parameters for both the mixture kernel and the mixture weights can be associated with a continuation-ratio logits regression structure. Hence, an efficient and relatively easy to implement posterior simulation method can be designed, using P\'olya-Gamma data augmentation. Moreover, the model is built from a conditional independence structure for category-specific parameters, which results in additional computational efficiency gains through partial parallel sampling. In addition to the general mixture structure, we study simplified model versions that incorporate covariate dependence only in the mixture kernel parameters or only in the mixture weights. For all proposed models, we discuss approaches to prior specification and develop Markov chain Monte Carlo methods for posterior simulation. The methodology is illustrated with several synthetic and real data examples.

==> chapter5.tex <==
\section{Models accounting for overdispersion}
\label{sec:overdmodel}

\subsection{General model formulation and properties}
\label{subsec:modformoverd}

Accounting for the extended ordinal regression problem, that is, when $m>1$, to model the possible intracluster correlation, we consider the overdispersed version of the models. One of the virtues of our model formulation is that it enables straightforward extension to incorporate overdispersion. Since we have factorized the multinomial distribution into product of binomial distributions, we can just replace the binomial distributions with logistic-normal binomial distributions to achieve overdispersion. Specifically, extending the general model, we define the general covariate-dependent nonparametric model for extended ordinal regression problem as
\begin{equation}
    \begin{split}
        &\mathbf{Y}|G_{\mathbf{x}}\stackrel{ind.}{\sim}\int\prod_{j=1}^{C-1}[\int Bin(Y_j|m_j,\varphi(\phi_j))N(\phi_j|\theta_j,\sigma_j^2)d\phi_j]dG_{\mathbf{x}}(\boldsymbol{\theta})\\
        &G_{\mathbf{x}}|\boldsymbol{\gamma}_0,\Gamma_0,\boldsymbol{\psi}\sim LSBP(\boldsymbol{\gamma}_0,\Gamma_0,G_{0\mathbf{x}}),\,\, \sigma_j^2\stackrel{i.i.d.}{\sim}IG(\sigma_j^2|a_{\sigma},b_{\sigma})
    \end{split}
    \label{eq:overdgeneralmodel}
\end{equation}
where $G_{0\mathbf{x}}$ defined exactly the same as in (\ref{eq:generalmodori}). $\theta_j=\mathbf{x}^T\boldsymbol{\beta}_j,j=1,\cdots,C-1$ and $\boldsymbol{\psi}$ represents the collection of parameters $\{\boldsymbol{\mu}_j,\Sigma_j\}_{j=1}^{C-1}$ in $G_{0\mathbf{x}}$. The model is complete with prior on $\boldsymbol{\psi}$:
\begin{equation}
    \boldsymbol{\mu}_j|\Sigma_j\stackrel{ind.}{\sim}N(\boldsymbol{\mu}_j|\boldsymbol{\mu}_{0j},\Sigma_j/\kappa_{0j}),\,\, \Sigma_j\stackrel{ind.}{\sim}IW(\Sigma_j|\nu_{0j},\Lambda_{0j}^{-1})
\end{equation}
Written in the infinite mixture model framework, 
\begin{equation}
  \mathbf{Y}|G_{\mathbf{x}}\stackrel{ind.}{\sim}\sum_{\ell=1}^{\infty}\omega_{\ell\mathbf{x}}\prod_{j=1}^{C-1}\int Bin(Y_j|m_j\varphi(\phi_j))N(\phi_j|\mathbf{x}^T\boldsymbol{\beta}_{j\ell},\sigma_j^2)d\phi_j
  \label{eq:overdinfsumform}
\end{equation}
where the weights are generated by the logit stick-breaking process: $\omega_{1\mathbf{x}}=\varphi(\mathbf{x}^T\boldsymbol{\gamma}_1)$ and $\omega_{\ell\mathbf{x}}=\varphi(\mathbf{x}^T\boldsymbol{\gamma}_{\ell})\prod_{h=1}^{\ell-1}(1-\varphi(\mathbf{x}^T\boldsymbol{\gamma}_h))$, $\ell=2,3,\cdots$ and $\boldsymbol{\gamma}_{\ell}\stackrel{i.i.d.}{\sim}N(\boldsymbol{\gamma}_{\ell}|\boldsymbol{\gamma}_0,\Gamma_0),\forall \ell\in\mathbb{N}_+$. The atoms $\boldsymbol{\beta}_{j\ell}\stackrel{i.i.d.}{\sim}N(\boldsymbol{\beta}_{j\ell}|\boldsymbol{\mu}_j,\Sigma_j)$, for $j=1,\cdots,C-1$. Comparing with the previous model (\ref{eq:infmixgeneralmodel}), the only difference is that we replace the mixing kernel with the logistic-normal-binomial distribution. 

Since there is only minor modification between the model (\ref{eq:generalmodori}) and the model (\ref{eq:overdgeneralmodel}), the latter one inherits most of the properties of the former as discussed in Section \ref{subsec:modpropori}, with modification applied. For example, under the model (\ref{eq:overdgeneralmodel}), we can still achieve flexible ordinal regression relationships, with the marginal probability response curves defined as
\begin{equation}
    Pr(\mathbf{Y}=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)=\sum_{\ell=1}^{\infty}\omega_{\ell\mathbf{x}}\{(\int\varphi(\phi_j)N(\phi_j|\theta_{j\ell\mathbf{x}},\sigma_j^2)d\phi_j)\prod_{k=1}^{j-1}[\int(1-\varphi(\phi_k))N(\phi_k|\theta_{k\ell\mathbf{x}},\sigma_k^2)d\phi_k]\}
    \label{eq:marproboverdmodel}
\end{equation}
In addition, suppose $\mathbf{Y}=\sum_{l=1}^m\tilde{\mathbf{Y}}_l$, where $\tilde{\mathbf{Y}}_l=(\tilde{Y}_{l1},\cdots,\tilde{Y}_{lC})$ satisfies $\sum_{j=1}^C\tilde{Y}_{lj}=1$. Denote the probability of $\mathbf{Y}$ taking category $j$ as $\pi_j$, we have
\begin{equation}
\begin{split}
    E(\pi_j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)&=E(\tilde{\mathbf{Y}}_l=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)\\
    &=\sum_{\ell=1}^{\infty}\omega_{\ell\mathbf{x}}\{(\int\varphi(\phi_j)N(\phi_j|\theta_{j\ell\mathbf{x}},\sigma_j^2)d\phi_j)\prod_{k=1}^{j-1}[\int(1-\varphi(\phi_k))N(\phi_k|\theta_{k\ell\mathbf{x}},\sigma_k^2)d\phi_k]\}\\
    Var(\pi_j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)&=Var(\tilde{\mathbf{Y}}_l=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)=E(\tilde{\mathbf{Y}}_l=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)-[E(\tilde{\mathbf{Y}}_l=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)]^2
\end{split}
\label{eq:momoverdmodel}
\end{equation}
As a consequence, the variance of $\mathbf{Y}$ is given by
\begin{equation}
    \begin{split}
        Var(\mathbf{Y}=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)&=m(m-1)Var(\pi_j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)+mVar(\tilde{Y}_l=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)\\
        &\geq mVar(\tilde{Y}_l=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)
    \end{split}
    \label{varoverdy}
\end{equation}
where the last line is the variance when $\tilde{\mathbf{Y}}_l$s are independent. Therefore, the model achieves overdispersion. Another important property of the overdispersed model is its capability to model the possible intracluster correlation, we have
\begin{equation}
\begin{split}
    Cov(\tilde{Y}_{jl},\tilde{Y}_{jl'}|G_{\mathbf{x}},\boldsymbol{\sigma}^2)&=Cov(E(\tilde{Y}_{jl}|\pi_j),E(\tilde{Y}_{jl'}|\pi_j)|G_{\mathbf{x}},\boldsymbol{\sigma}^2)+E(Cov(\tilde{Y}_{jl},\tilde{Y}_{jl'}|\pi_j)|G_{\mathbf{x}},\boldsymbol{\sigma}^2)\\
    &=Var(\pi_j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)
\end{split}    
    \label{eq:covoverdmodel}
\end{equation}

We shall also mention that this overdispersed model has a drawback, that is, the integral of the logistic normal distribution in general do not have analytical form. Therefore, in practice when we fit this model and do the inference, we need a good numerical method to approximate the integral. Fortunately, that method exists. It turns out that a simple Riemann sum can approximate the integral efficiently, with error controlled. Specifically, to approximate a logistic normal integral $\int \varphi(\phi)N(\phi|\mu,\sigma^2)d\phi$, based on experience, we can set $N=500$ equally spaced points $\tilde{\phi}_i$ in the region $(\mu-4\sigma,\mu+4\sigma)$. Then the Reimann sum $8\sigma/N\sum_{i=1}^N\varphi(\tilde{\phi}_i)N(\tilde{\phi}_i|\mu,\sigma^2)$ can approximate the original integral.  

To complete the model, we use conjugate prior for the model parameters, that is,
\begin{equation}
    \boldsymbol{\gamma}_{\ell}\stackrel{i.i.d.}{\sim} N(\boldsymbol{\gamma}_{\ell}|\boldsymbol{\gamma}_0,\Gamma_0),\,\, \boldsymbol{\mu}_j|\Sigma_j\stackrel{ind.}{\sim}N(\boldsymbol{\mu}_j|\boldsymbol{\mu}_{0j},\Sigma_j/\kappa_{0j}),\,\, \Sigma_j\stackrel{ind.}{\sim}IW(\Sigma_j|\nu_{0j},\Lambda_{0j}^{-1}),\,\, \sigma_j^2\stackrel{i.i.d.}{\sim} IG(\sigma_j^2|a_{\sigma},b_{\sigma})
    \label{eq:priorsepcgenoverd}
\end{equation}
An conventional choice for the hyperparameters would be to apply the baseline choice of prior hyperparameters from the original model, and further assume $a_{\sigma}=b_{\sigma}=1$. Using proposition \ref{prop:baselinelogitnormal}, the probability response curves under the overdispersed model with the  baseline choice of hyperparameters are again given by $E(Pr(\mathbf{Y}=j|G_{\mathbf{x}}))=2^{-j}$ for $j=1,\cdots,C-1$ and $E(Pr(\mathbf{Y}=C|G_{\mathbf{x}}))=2^{-(C-1)}$, with a wide enough variation that covers the whole unit interval. 

Inspired by specific applications, such as the developmental toxicity study example we will discuss in Section \ref{sec:overdexample}, sometimes we have to carefully tuning the prior hyperparameters to reflect our strong prior belief on the regression functional $Pr(\mathbf{Y}|\mathbf{x})$. Such prior information is usually about the monotonicity of the regression functional on a certain region. Using proposition \ref{prop:logitnormalexpbound}, it is not hard to see the prior hyperparameters such that the expected regression functionals under the original model have certain types of monotonicity will keep the same type of monotonicity under the overdispersed model. Therefore, to achieve certain type of monotonicty, we will use the same strategy proposed in Section \ref{subsec:prispecori}. The hyperparameter $a_{\sigma}$ and $b_{\sigma}$ controls the variability of overdispersed parameter. We set $a_{\sigma}=b_{\sigma}=1$ to in favor a relatively large variation. As an example, we plot the prior expected regression functionals and five prior realizations under using the same prior hyperparameters as in Figure \ref{fig:priorpiest}. The result is shown in Figure \ref{fig:priorpiestoverd}.

\begin{figure}
\centering
\includegraphics[width=16cm,height=8cm]{specprioroverd.png}
\caption{Prior specification under the overdispersed model with the same prior hyperparameters as before. The red solid line is the prior expected probability response curves. The blue dashed lines and shaded regions are the prior $95\%$ interval estimate, while the green dotted lines are 5 prior realizations.}
\label{fig:priorpiestoverd}
\end{figure}


An appealing feature of this modeling approach to encounter overdispersion is that the computational method is extremely easily to develop. With the posterior inference algorithm for the original general model at hand, we only need tiny modification to make that algorithm works for the overdispersed general model. That is, we can apply a Gibbs sampler to simulate posterior samples of all model parameters for the overdispersed model, with all full conditional distributions known in explicit form and easy to sample from. The computation for the overdispersed model is also efficient.  

To be specific, for each $\mathbf{Y}_i$, we introduce the same two groups of Pólya-Gamma latent variables as we do for the original general model. Then the overdispersed model is just adding one more layer to (\ref{eq:blockedgibbsgeneral})
\begin{equation}
\begin{split}
    &\mathbf{Y}_i|\boldsymbol{\phi}_i,\boldsymbol{\zeta}_i\stackrel{ind.}{\sim}\prod_{j=1}^{C-1}\exp\{(y_{ij}-\frac{m_{ij}}{2})\phi_{ij}-\frac{\zeta_{ij}}{2}\phi_{ij}^2\}\\
    &\zeta_{ij}\sim PG(\zeta_{ij}|m_{ij},0),\,\, \phi_{ij}|\boldsymbol{\mathcal{L}}_i,\boldsymbol{\beta}\sim N(\phi_{ij}|\mathbf{x}_i^T\boldsymbol{\beta}_{j\mathcal{L}_i},\sigma_j^2)\,\,
    \boldsymbol{\beta}_{j\ell}|\boldsymbol{\mu}_j,\Sigma_j\sim N(\boldsymbol{\beta}_{j\ell}|\boldsymbol{\mu}_j,\Sigma_j)\\
    &\mathcal{L}_i\Longleftrightarrow\boldsymbol{\mathcal{L}}_i,\,\, \boldsymbol{\mathcal{L}}_i|\boldsymbol{\gamma},\boldsymbol{\xi}_i\stackrel{ind.}{\sim}\prod_{\ell=1}^{L-1}\exp\{(\mathcal{L}_{i\ell}-\frac{\tilde{m}_{i\ell}}{2})\mathbf{x}_i^T\boldsymbol{\gamma}_{\ell}-\frac{\xi_{i\ell}}{2}(\mathbf{x}_i^T\boldsymbol{\gamma}_{\ell})^2\},\,\, \zeta_{ij}\sim PG(\zeta_{ij}|m_{ij},0)\\
    &\boldsymbol{\gamma}_{\ell}\stackrel{i.i.d.}{\sim} N(\boldsymbol{\gamma}_{\ell}|\boldsymbol{\gamma}_0,\Gamma_0),\,\, \boldsymbol{\mu}_j|\Sigma_j\stackrel{ind.}{\sim} N(\boldsymbol{\mu}_j|\boldsymbol{\mu}_{0j},\Sigma_j/\kappa_{0j}),\,\, \Sigma_j\stackrel{ind.}{\sim}IW(\Sigma_j|\nu_{0j},\Lambda_{0j}^{-1})\,\, \sigma_j^2\sim IG(\sigma_j^2|a_{\sigma},b_{\sigma})
\end{split}
\label{eq:blockedgibbsgeneraloverd}
\end{equation}
Proceeding to the exact steps of the blocked Gibbs sampler, we let $n^*$ and $M_{\ell}$ to have the same meaning as previous, the blocked Gibbs sampler for the overdispersed general model is based on simulation from the following posterior full conditional distributions. This algorithm is adapted from the blocked Gibbs sampler proposed in Section \ref{subsec:postinfori}, with modification to include the update of latent variable $\phi_{ij}$ and overdispersed parameter $\sigma_j^2$, which are introduced by using the overdispersed kernel. 

\noindent\textbf{Step 1: update latent variables $\phi_{ij}$.} Conditioning on all other variables, the update of $\phi_{ij}$ uses the standard normal normal conjugacy. That is, for $i=1,\cdots,n,j=1,\cdots,C-1$ and $m_{ij}>0$, we update $\phi_{ij}$ by sample from $N(\phi_{ij}|\tilde{\theta}_{ij},\tilde{\sigma}^2_{ij})$ with parameter $\tilde{\theta}_{ij}=\mathbf{x}_i^T\boldsymbol{\beta}_{j\mathcal{L}_i}+\sigma_j^2(y_{ij}-m_{ij}/2)/(1+\sigma_j^2\zeta_{ij})$ and $\tilde{\sigma}^2_{ij}=\sigma_j^2/(1+\sigma_j^2\zeta_{ij})$. 


\noindent\textbf{Step 2: update parameters in the atoms.} In this step, we update two sets of parameters, $\{\boldsymbol{\beta}_{j\ell}:j=1,\cdots,C-1,\ell=1,\cdots,L\}$ and $\{\zeta_{ij}:i=1,\cdots,n,j=1,\cdots,C-1,\zeta_{ij}\neq 0\}$. Since we add a latent layer such that $\boldsymbol{\beta}_{j\ell}$ depends on $\phi_{ij}$ instead of $Y_{ij}$, we only need to modify the updating steps that involves $y_{ij}$. Therefore, when there exist $i$ satisfies  $\mathcal{L}_i=\mathcal{L}_r^*$ for some $r\in\{1,\cdots,n^*\}$,  and $m_{ij}\neq 0$, $\boldsymbol{\beta}_{j\ell}$ is drawn from multivariate normal distribution $N(\cdot|\tilde{\boldsymbol{\mu}}_j,\tilde{\Sigma}_j)$ with updated scale parameter $\tilde{\Sigma}_j=(X_{\mathcal{L}_r^*}^TX_{\mathcal{L}_r^*}/\sigma_j^2+\Sigma_j^{-1})^{-1}$ and location parameter $\tilde{\boldsymbol{\mu}}_j=\tilde{\Sigma}_j(X_{\mathcal{L}_r^*}^T\boldsymbol{\phi}_{\mathcal{L}_r^*j}+\Sigma_j^{-1}\boldsymbol{\mu}_j)$, where $X_{\mathcal{L}_r^*}$ is the matrix whose row vectors are given by $\mathbf{x}_i$, and $\boldsymbol{\phi}_{\mathcal{L}_r^*j}$ is the vector of $\phi_{ij}$ where $i$ need to satisfies $\mathcal{L}_i=\mathcal{L}_r^*,m_{ij}\neq0$. The other updating in this step is the same as for the general model.


\noindent\textbf{Step 3: update parameters in the weights.} Since we have the same structure for the weights as the original model, this updating step is exactly the same as before.

\noindent\textbf{Step 4: update configuration variables.} Because the configuration variables depend on $\phi_{ij}$ instead of $Y_{ij}$, we have now the $\tilde{p}_{i\ell}\propto p_{i\ell}\prod_{j=1}^{C-1}N(\phi_{ij}|\mathbf{x}^T_{i}\boldsymbol{\beta}_{j\ell},\sigma_j^2)$. The $p_{i\ell}$ is defined the same as before. 

\noindent\textbf{Step 5: update overdispersion parameters.} Since the model include a set of overdispersion parameters $\sigma^2_j$, we add this step to update them in each iteration. Due to conjugacy, the full conditional distribution is $\sigma_j^2\sim IG(\sigma_j^2|a_{\sigma}^*,b_{\sigma j}^*)$, where $a_{\sigma}^*=a_{\sigma}+n_j/2$ and $b_{\sigma j}^*=b_{\sigma}+\sum_{i=1}^n(\phi_{ij}-\mathbf{x}_i^T\boldsymbol{\beta}_{j\mathcal{L}_i})^2/2$, where $n_j$ is the number of $m_{ij}\neq 0$. 

\noindent\textbf{Step 6: update hyperparameters.}  The updating of hyperparameters $\{\boldsymbol{\mu}_j,\Sigma_j\}$ are also exactly the same as before. 


With the samples of all model parameters obtained from the full posterior distribution, we are able to perform inference on quantities of interest. Similar as before, let the superscript $(t)$ denote the $t-$th posterior sample of parameter. At the $t-$th MCMC iteration, the regression functional $Pr(\mathbf{Y}=j|G_{\mathbf{x}})$ can be compute over a grid in $\mathcal{X}$ via
\begin{equation}
\begin{split}
   Pr(\mathbf{Y}=j|G_{\mathbf{x}})&=\sum_{\ell=1}^{L}\{\varphi(\mathbf{x}^T\boldsymbol{\gamma}_{\ell}^{(t)})\prod_{h=1}^{\ell-1}[1-\varphi(\mathbf{x}^T\boldsymbol{\gamma}_{h}^{(t)})]\}\\
   &\times\{[\int\varphi(\phi_j)N(\phi_j|\mathbf{x}^T\boldsymbol{\beta}_{j\ell}^{(t)},(\sigma^2_j)^{(t)})d\phi_j]\prod_{k=1}^{j-1}[\int(1-\varphi(\phi_k))N(\phi_k|\mathbf{x}^T\boldsymbol{\beta}_{k\ell}^{(t)},(\sigma^2_j)^{(t)})d\phi_k]\}
\end{split}   
    \label{eq:margcurvepostoverd} 
\end{equation}
for $j=1,\cdots,C$. The $t-$th posterior predictive sample of $\mathbf{Y}_*$ with a new covariate $\mathbf{x}_*$ can be obtained by first sample the corresponding configuration variable $\mathcal{L}^{(t)}_*$ from the discrete distribution on $\{1,\cdots,L\}$ with $Pr(\mathcal{L}^{(t)}_*=\ell)=\varphi(\mathbf{x}^T\boldsymbol{\gamma}_{\ell}^{(t)})\prod_{h=1}^{\ell-1}[1-\varphi(\mathbf{x}^T\boldsymbol{\gamma}_{h}^{(t)})]$, $\ell=1,\cdots,L-1$ and $Pr(\mathcal{L}^{(t)}_*=L)=\prod_{\ell=1}^{L-1}[1-\varphi(\mathbf{x}^T\boldsymbol{\gamma}_{\ell}^{(t)})]$, then sample latent variable $\boldsymbol{\phi}^{(t)}_*$ from $\prod_{j=1}^{C-1}N(\phi^{(t)}_{*j}|\mathbf{x}^{T}_*\boldsymbol{\beta}_{j\mathcal{L}^{(t)}_*}^{(t)},(\sigma_j^2)^{(t)})$, and finally get the posterior predictive sample $\mathbf{Y}^{(t)}$ from $\prod_{j=1}^{C-1}Bin(Y^{(t)}_{*j}|m_{*j},\varphi(\phi^{(t)}_{*j}))$. After the computation at each iteration, we attain the posterior point and interval estimate of these quantities by standard Monte Carlo estimate. 


\subsection{Simplified model with linear DDP prior}
\label{subsec:overdlddpmodel}

As a simpler model for the extended ordinal regression problem would be to allow only the atoms in the infinite mixture prior to depend on the covariates, of which an obvious choice would be the linear DDP prior. This model is an extension of the linear DDP model we have discussed in Section \ref{sec:orimodel}. The model is given as
\begin{equation}
    \begin{split}
        &\mathbf{Y}|G_{\mathbf{x}}\stackrel{ind.}{\sim}\int\prod_{j=1}^{C-1}[\int Bin(Y_j|m_j,\varphi(\phi_j))N(\phi_j|\theta_j,\sigma_j^2)d\phi_j]dG_{\mathbf{x}}(\boldsymbol{\theta})\\
        &G_{\mathbf{x}}|\alpha,\boldsymbol{\psi}\sim DDP(\alpha,G_{0\mathbf{x}}),\,\, \sigma_j^2\stackrel{i.i.d.}{\sim}IG(\sigma_j^2|a_{\sigma},b_{\sigma})\\
        &\alpha\sim Gamma(\alpha|a_{\alpha},b_{\alpha}),\quad \boldsymbol{\mu}_j|\Sigma_j\stackrel{ind.}{\sim} N(\boldsymbol{\mu}_j|\boldsymbol{\mu}_{0j},\Sigma_j/\kappa_{0j}),\quad \Sigma_j\stackrel{ind.}{\sim}IW(\Sigma_j|\nu_{0j},\Lambda_{0j}^{-1})
    \end{split}
    \label{eq:overdlddpmodel}
\end{equation}

Similar as the gereral case, the linear DDP model also achieves overdispersion, since comparing with the general case, the linear DDP model only uses different stick-breaking weights. Furthermore, we lose some generality in ordinal regression relationships, with the marginal probability response curves now given by
\begin{equation}
    Pr(\mathbf{Y}=j|G_{\mathbf{x}},\boldsymbol{\sigma}^2)=\sum_{\ell=1}^{\infty}\omega_{\ell}\{(\int\varphi(\phi_j)N(\phi_j|\theta_{j\ell\mathbf{x}},\sigma_j^2)d\phi_j)\prod_{k=1}^{j-1}[\int(1-\varphi(\phi_k))N(\phi_k|\theta_{k\ell\mathbf{x}},\sigma_k^2)d\phi_k]\}
    \label{eq:marproboverdlddpmodel}
\end{equation}
where the weights $\omega_l$ are generated by the stick-breaking process with breaking proportion generated from $Beta(1,\alpha)$. To specify the prior hyperparameters, we can apply the same strategy as the general model, with the hyperparameters $a_{\alpha},b_{\alpha}$ been specified with the consideration about the distinct component. 

The benefit of the linear DDP model is that it release the computation burden of the posterior inference. After introducing the same set of latent variables as in the general case, the same blocked Gibbs sampler can be used, with the steps about updating parameters that related to weights been changed. Specifically, we replace the steps about updating parameters in the weights and updating configuration variables with the following

\noindent\textbf{Step 3: update configuration variables.} In this step, we first sample $V_{\ell}^*\stackrel{ind.}{\sim}Beta(V_{\ell}^*|1+M_{\ell},\alpha+\sum_{h=\ell+1}^LM_h)$ for $\ell=1,\cdots,L-1$, and then let $p_1=V_1^*$, $p_{\ell}=V_{\ell}^*\prod_{h=1}^{\ell-1}(1-V_h^*)$ for $\ell=2,\cdots,L-1$ and $p_L=1-\sum_{\ell=1}^{L-1}p_{\ell}$. Finally to update the configuration variable $L_i$, we sample it from the discrete distribution on $\{1,\cdots,L\}$ with probability that $L_i=\ell$ satisfies $\tilde{p}_{i\ell}\propto p_{i\ell}\prod_{j=1}^{C-1}N(\phi_{ij}|\mathbf{x}^T_{i}\boldsymbol{\beta}_{j\ell},\sigma_j^2)$. 


\noindent\textbf{Step 4: update parameters in the weights.} We update $\alpha$ by sample from $Gamma(\alpha|a_{\alpha}+L-1,b_{\alpha}-\sum_{h=1}^{L-1}\log(1-V_h^*))$.




==> chapter6.tex <==
{\color{blue}
\section{On the support of the proposed models}
\label{sec:fullsupport}

In this section we establish the full support property of our proposed models for ordinal response distributions. The density neighborhoods are defined by the Kullback-Leibler (KL) divergence. We claim the general model and its two simplifications all possess the KL property. 


}
